Unsupervised Deep Manifold Attributed Graph Embedding

Unsupervised attributed graph representation learning is challenging since both structural and feature information are required to be represented in the latent space. Existing methods concentrate on learning latent representation via reconstruction tasks, but cannot directly optimize representation and are prone to oversmoothing, thus limiting the applications on downstream tasks. To alleviate these issues, we propose a novel graph embedding framework named Deep Manifold Attributed Graph Embedding (DMAGE). A node-to-node geodesic similarity is proposed to compute the inter-node similarity between the data space and the latent space and then use Bergman divergence as loss function to minimize the difference between them. We then design a new network structure with fewer aggregation to alleviate the oversmoothing problem and incorporate graph structure augmentation to improve the representation's stability. Our proposed DMAGE surpasses state-of-the-art methods by a significant margin on three downstream tasks: unsupervised visualization, node clustering, and link prediction across four popular datasets.

==> Tab_result_ssl_STL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% table_ch_4_3
\begin{table}[!htbp]
    \centering
    \caption{Visual representation learning performance on STL-10}
    {
        % \footnotesize
    % {\scriptsize
    \begin{tabular}{lcccccc}
    \toprule
                & \multicolumn{2}{c}{400 ep} & \multicolumn{2}{c}{800 ep} & \multicolumn{2}{c}{1600 ep} \\
                & top 1        & top 5       & top 1        & top 5       & top 1        & top 5        \\ \midrule
    Related-loc & 56.26        & 95.25       & 59.49        & 96.45       & -            & -            \\
    Rotation    & 76.04        & 99.40       & 70.57        & 98.86       & -            & -            \\
    NPID        & 82.28        & 99.33       & 83.93        & 99.39       & 89.45        & 99.59        \\
    ODC         & 72.51        & 98.78       & 76.16        & 98.68       & 77.84        & 98.69        \\
    SimCLR      & 86.92        & 99.01       & 87.66        & 98.98       & 89.25        & 99.47        \\
    MoCo.v2     & 85.53        & 99.55       & 89.26        & 99.58       & 91.29        & 99.46        \\
    BYOL        & 81.11        & 99.38       & 88.55        & 99.54       & 91.46        & 99.54        \\
    G-ELIS      & 88.31        & 99.55       & 91.02        & 99.63       & 91.45        & 99.65        \\
    \bottomrule
    \label{Tab_result_ssl_STL}
    \end{tabular}}
\end{table}


==> __latexindent_temp.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
    \centering
    {
        % \footnotesize
        \caption{Node clustering performance on PubMed, Cora, CiteSeer and Wiki}
        \begin{tabular}{@{}cc|ccc|ccc|ccc|ccc@{}}
            \toprule
            \multirow{2}{*}{Method}                          & \multirow{2}{*}{Input}     & \multicolumn{3}{c|}{\pmb{CORA}}                & \multicolumn{3}{c|}{\pmb{CiteSeer}}          & \multicolumn{3}{c|}{\pmb{PubMed}}            & \multicolumn{3}{c}{\pmb{Wiki}}                      \\ 
                                                             &                            & ACC           & NMI           & F1            & ACC           & NMI           & F1            & ACC           & NMI           & F1           & ACC           & NMI           & F1            \\ \midrule
            k-means                                          & Feature                    & 34.7          & 16.7          & 25.4          & 38.5          & 17.0          & 30.5          & 57.3          & 29.1          & 57.4         & 33.4          & 30.2          & 24.5          \\
            Spectral-f                                       & Feature                    & 36.3          & 15.1          & 25.6          & 46.2          & 21.2          & 33.7          & 59.9          & 32.6          & 58.6         & 41.3          & 44.0          & 25.2          \\ \midrule
            Spectral-g                                       & Graph                      & 34.2          & 19.5          & 30.2          & 25.9          & 11.8          & 29.5          & 39.7          & 3.5           & 52.0         & 23.6          & 19.3          & 17.2          \\
        DeepWalk(2014) {\cite{perozzi_deepwalk_2014}}        & Graph                      & 46.7          & 31.8          & 38.1          & 36.2          & 9.7           & 26.7          & 61.9          & 16.7          & 47.1         & 38.5          & 32.4          & 25.7          \\
            DNGR(2016) {\cite{cao_deep_2016}}                & Graph                      & 49.2          & 37.3          & 37.3          & 32.6          & 18.0          & 44.2          & 45.4          & 15.4          & 17.9         & 37.6          & 35.9          & 25.4          \\ \midrule
            GAE(2016) {\cite{kipf_variational_2016}}         & Both                       & 53.3          & 40.7          & 42.0          & 41.3          & 18.3          & 29.1          & 64.1          & 23.0          & 49.3         & 17.3          & 11.9          & 15.4          \\
            VGAE(2016) {\cite{kipf_variational_2016}}        & Both                       & 56.0          & 38.5          & 41.5          & 44.4          & 22.7          & 31.9          & 65.5          & 25.1          & 51.0         & 28.7          & 30.3          & 20.5          \\
            MGAE(2017) {\cite{wang_mgae_2017}}               & Both                       & 63.4          & 45.6          & 38.0          & 63.6          & 39.8          & 39.5          & 43.9          & 8.2           & 42.0         & 50.1          & 48.0          & 39.2          \\
            ARGE(2018) {\cite{pan_adversarially_2018}}       & Both                       & 64.0          & 44.9          & 61.9          & 57.3          & 35.0          & 54.6          & 59.1          & 23.2          & 58.4         & 41.4          & 39.5          & 38.3          \\
          % ARVGE                                            & Both                       & 63.8          & 45.0          & 62.7          & 54.4          & 26.1          & 52.9          & 58.2          & 20.6          & 23.0         & 41.6          & 40.0          & 37.8          \\
            DANE(2018) {\cite{gao_deep_2018}}                & Both                       & 70.3          & 54.3          & 66.8          & 48.0          & 25.6          & 34.8          & 69.4          & 31.2          & 67.58        & 47.3          & 46.2          & 35.9          \\
            DGI (2018) {\cite{velickovic_deep_2018}}         & Both                       & 71.3          & 56.4          & 68.2          & 68.8          & 44.4          & 65.7          & 53.3          & 18.1          & 18.6         & -             & -             & -             \\
            AGC (2019) {\cite{zhang_attributed_2019}}        & Both                       & 68.9          & 53.7          & 65.6          & 67.0          & 41.1          & 62.5          & 69.8          & 31.6          & 68.7         & 47.7          & 45.2          & 35.7          \\
            DAEGC(2019) {\cite{wang_attributed_2019}}        & Both                       & 70.4          & 52.8          & 68.2          & 67.2          & 39.7          & 63.6          & 67.1          & 26.6          & 65.9         & -             & -             & -             \\
            ARGA(2020) {\cite{pan_learning_2020}}            & Both                       & 71.1          & 52.6          & 69.3          & 58.1          & 33.8          & 52.5          & 69.0          & 29.0          & 67.8         & -             & -             & -             \\
            AGE (2020) {\cite{cui_adaptive_2020}}            & Both                       & 71.2          & 55.9          & 68.2          & 56.9          & 34.8          & 54.4          & -             & -             & -            & 51.9          & 49.4          & 40.8          \\
\color{olivine}{GIC (2020){ \cite{mavromatis_graph_2020}} }  & \color{olivine}Both        &\color{olivine} 72.5 & \color{olivine} 53.7    & \color{olivine} 69.4          &\color{olivine} 69.6          &\color{olivine} \pmb{45.3}    &\color{olivine} 65.4          &\color{olivine} 67.3          &\color{olivine} 31.9          &\color{olivine} 70.4         &\color{olivine} 50.5          &\color{olivine} 48.6          &\color{olivine} 43.8          \\ \midrule
            Ours(DMAGE-SED)                                  & Both                       & {74.2}        & {58.0}        & {69.8}        & {69.6}        & 44.1          & {66.3}        & {73.3}        & {35.8}        & {73.2}       & {52.3}        & {49.0}        & {46.8}       \\ 
            Ours(DMAGE-LOGI)                                 & Both                       & \pmb{74.3}    & {57.7}        & {69.7}        & {69.7}        & 43.8          & {66.3}        & \pmb{76.0}    & \pmb{36.8}    & \pmb{75.8}   & \pmb{53.8}    & \pmb{50.4}    & \pmb{47.6}   \\ 
            Ours(DMAGE-SED+LOGI)                             & Both                       & \pmb{74.3}    & \pmb{58.2}    & \pmb{70.0}    & \pmb{69.9}    & 43.5          & \pmb{66.5}    & {74.1}        & {36.0}        & {73.1}       & 52.1          & {50.0}        & {44.6}       \\ \bottomrule
            \end{tabular}
        \label{Tab_result_node_clustering}
    }
\end{table*}

